Adaptively Pruning Features for Boosted Decision Trees

Boosted decision trees enjoy popularity in a variety of applications; however, for large-scale datasets, the cost of training a decision tree in each round can be prohibitively expensive. Inspired by ideas from the multi-arm bandit literature, we develop a highly efficient algorithm for computing exact greedy-optimal decision trees, outperforming the state-of-the-art Quick Boost method. We further develop a framework for deriving lower bounds on the problem that applies to a wide family of conceivable algorithms for the task (including our algorithm and Quick Boost), and we demonstrate empirically on a wide variety of data sets that our algorithm is near-optimal within this family of algorithms. We also derive a lower bound applicable to any algorithm solving the task, and we demonstrate that our algorithm empirically achieves performance close to this best-achievable lower bound.

==> boosting.tex <==
Boosting algorithms, e.g. AdaBoost, gradient boosting, LogiBoost etc, train a linear classifier $\mathcal{H}_T(x)=\sum^T_t {\alpha_t h_t(x)}$, where $h_t(x)$ is the weak learner selected at round $t$ such that an error function $\mathcal{E}_t$ is minimized, and $\alpha_t$ is an scaler optimized based on $\mathcal{E}_t$. Based on $\mathcal{E}_t$, each instance $x_i$ is assigned a weight $w_i$ such that instances misclassified at round $t$ are assigned heavier weights so that in the next round the algorithm focuses on these heavy weight instances when training weak learner $h_{t+1}(x)$. Decision Trees are often trained as weak learners.

\subsection{Decision Tree}

\begin{algorithm}[H]
\caption{SP-Boosting}\label{boosting}
\begin{algorithmic}
   \STATE {\bfseries Input:} Instances \{$x_1, \dots, x_n$\}, Labels \{$y_1, \dots, y_n$\}
   \STATE {\bfseries Output:} $\mathcal{H}_T(x)$
   \STATE {\bfseries Initialize Weights:} $\{w_{1},\dots,w_{n}\}$   \FOR{$t=1$ {\bfseries to} $T$}
   \STATE Train Decision Tree $h_t(x)$
   \STATE Choose $\alpha_t$
   \STATE $\mathcal{H}_t(x)=\mathcal{H}_{t-1}(x) + \alpha_t h_t(x)$
   \STATE Update and Sort (in descending order) $w$
   \ENDFOR
\end{algorithmic}
\end{algorithm}

==> figures/result2_table.tex <==
\begin{table*}[t]
\caption{Total Assessments after 500 rounds}
\label{tbl:pulls-at-depth}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llccccc}
\toprule
 &  & 1 & 2 & 3 & 4 & 5\\
\midrule
A6A & AP Boost & 6.40e+08 & 1.23e+09 & 1.69e+09 & 2.08e+09 & 2.44e+09 \\
A6A & Quick Boost & 6.66e+08 & 1.29e+09 & 1.83e+09 & 2.34e+09 & 2.89e+09 \\
W4A & AP Boost & 8.71e+08 & 1.38e+09 & 1.69e+09 & 1.90e+09 & 2.12e+09 \\
W4A & Quick Boost & 9.10e+08 & 1.72e+09 & 2.41e+09 & 3.07e+09 & 3.60e+09 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> table_results_approx.tex <==
\begin{table*}[ht]
\caption{Computational Complexity for LazyBoost and Boosting with Weight Trimming.
All results are for 500 rounds of boosting except MNIST (300 rounds) and RCV1 (400 rounds).}
\label{complexity-approx-results}	
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llccrccr}
\toprule
& & \multicolumn{3}{c}{CPU Time in Seconds} & \multicolumn{3}{c}{\# Example Assessments} \\
Dataset & Boosting & AP-B & QB & Improv. & AP-B & QB & Improv. \\
\midrule
a6a & LazyBoost (0.5) & 1.81e+02 & 2.02e+02 & 10.6\% & 8.53e+08 & 9.24e+08 & 7.7\% \\
a6a & LazyBoost (0.9) & 3.18e+02 & 3.53e+02 & 10.1\% & 1.52e+09 & 1.65e+09 & 7.9\% \\
a6a & Weight Trim (0.9) & 2.70e+02 & 2.76e+02 & 2.3\% & 1.19e+09 & 1.27e+09 & 6.4\% \\
a6a & Weight Trim (0.99) & 3.45e+02 & 3.25e+02 & -6.0\% & 1.57e+09 & 1.59e+09 & 1.2\% \\
\midrule
%
rcv1 & LazyBoost (0.5) & 8.39e+04 & 8.00e+04 & -4.9\% & 3.23e+11 & 3.33e+11 & 2.8\% \\
rcv1 & LazyBoost (0.9) & 1.53e+05 & 1.47e+05 & -4.0\% & 5.66e+11 & 5.90e+11 & 4.0\% \\
rcv1 & Weight Trim (0.9) & 9.58e+04 & 9.26e+04 & -3.5\% & 3.70e+11 & 3.73e+11 & 1.0\% \\
rcv1 & Weight Trim (0.99) & 1.54e+05 & 1.49e+05 & -3.8\% & 5.65e+11 & 5.77e+11 & 2.1\% \\
\midrule
%
satimage & LazyBoost (0.5) & 4.59e+02 & 5.35e+02 & 14.2\% & 5.13e+08 & 6.10e+08 & 15.8\% \\
satimage & LazyBoost (0.9) & 7.03e+02 & 8.66e+02 & 18.8\% & 7.96e+08 & 9.96e+08 & 20.1\% \\
satimage & Weight Trim (0.9) & 1.11e+03 & 1.09e+03 & -1.5\% & 1.26e+09 & 1.26e+09 & 0.0\% \\
satimage & Weight Trim (0.99) & 7.39e+02 & 7.60e+02 & 2.8\% & 7.07e+08 & 7.48e+08 & 5.5\% \\
\midrule
%
w4a & LazyBoost (0.5) & 1.21e+02 & 1.63e+02 & 25.5\% & 8.56e+08 & 1.23e+09 & 30.3\% \\
w4a & LazyBoost (0.9) & 2.05e+02 & 2.80e+02 & 26.9\% & 1.51e+09 & 2.17e+09 & 30.2\% \\
%w4a & Weight Trim (0.9) & 1.78e+02 & 1.76e+02 & -1.2\%  & 1.36e+09 & 1.41e+09 & 3.2\% \\
w4a & Weight Trim (0.9) & 2.51e+02 & 2.37e+02 & -6.0\% & 1.38e+09 & 1.34e+09 & -3.2\% \\
w4a & Weight Trim (0.99) & 2.47e+02 & 2.64e+02 & 6.6\% & 1.41e+09 & 1.54e+09 & 8.4\% \\
\midrule
Mean & (with rcv1)  & &  & X\% & & & X\% \\
\midrule
Mean & (without rcv1)  & &  & X\% & & & X\% \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


